Excitations in the Yang-Gaudin Bose gas

We study the excitation spectrum of two-component delta-function interacting bosons confined to a single spatial dimension, the Yang-Gaudin Bose gas. We show that there are pronounced finite-size effects in the dispersion relations of excitations, perhaps best illustrated by the spinon single particle dispersion which exhibits a gap at $2k_F$ and a finite-momentum roton minimum. Such features occur at energies far above the finite volume excitation gap, vanish slowly as $1/L$ for fixed spinon number, and can persist to the thermodynamic limit at fixed spinon density. Features such as the $2k_F$ gap also persist to multi-particle excitation continua. Our results show that excitations in the finite system can behave in a qualitatively different manner to analogous excitations in the thermodynamic limit. The Yang-Gaudin Bose gas is also host to multi-spinon bound states, known as $\Lambda$-strings. We study these excitations both in the thermodynamic limit under the string hypothesis and in finite size systems where string deviations are taken into account. In the zero-temperature limit we present a simple relation between the length $n$ $\Lambda$-string dressed energies $\epsilon_n(\lambda)$ and the dressed energy $\epsilon(k)$. We solve the Yang-Yang-Takahashi equations numerically and compare to the analytical solution obtained under the strong couple expansion, revealing that the length $n$ $\Lambda$-string dressed energy is Lorentzian over a wide range of real string centers $\lambda$ in the vicinity of $\lambda = 0$. We then examine the finite size effects present in the dispersion of the two-spinon bound states by numerically solving the Bethe ansatz equations with string deviations.

==> sh_continuum_strongcouplingexpansion.tex <==
%%%%%%%%%%%%%%% STRONG COUPLING EXPANSION FOR s\bar h continuum. 
\begin{comment}

%%%
\subsubsection{Strong coupling expansion.}
%%%
The strong coupling expansion starts from the integral equation for the shift function, as previously discussed. For the $s\bar h$ excitation, this reads 
\bea
\pi {\rm sgn}(j-j_1) &=& 2\pi F_{s\bar h}(k_j^{(0)}|k_h,\Lambda) - \phi_2(k_j^{(0)},\Lambda)\nn && - \int_{-q_L}^{q_R} \rd q F_{s\bar h}(q|k_h,\Lambda) K(k_j^{(0)},q),
\eea
and the spin rapidity satisfies
\be
2\pi J = L \int_{-q_L}^{q_R} \rd k \rho(k) \phi_2(\Lambda,k) + \int_{-q_L}^{q_R} \rd k F_{s\bar h}(k|k_h,\Lambda) \rho(k) \phi_2'(\Lambda,k).
\ee
The (possibly) non-symmetric bounds of the integral $q_L, q_R$ reflect the fact that the Fermi surface is not symmetric in the presence of the spinon (see Sec.~\ref{Sec:Spinon}). The shift function $F_{s\bar h}(k|k_h,\Lambda)$ quantifies the effect of adding the hole $k_h$ and the spin rapidity $\Lambda$ on the momenta. Following an expansion in $1/c$ we find the following
\bea
F_{s\bar h}(k_j|k_h,\Lambda) = \frac{1}{2\pi} \phi_2(k_j,\Lambda) + \frac{1}{2}\Xi(k-k_h)\Bigg[1 + \frac{1}{\pi c}(q_R + q_L) \Bigg]\nn
\hspace{2.5cm}+ \frac{1}{2\pi^2} \Bigg[ G\Bigg(\frac{2(q_R-\Lambda)}{c}\Bigg) - G\Bigg(\frac{2(q_L + \Lambda)}{c} \Bigg)\Bigg]+\ldots,\\ 
\rho(k) = \frac{1}{2\pi} + \frac{1}{2\pi^2 c}(q_R + q_L)+ \ldots,\\
q_R = \pi \varrho \Bigg( 1 - \frac{2}{c} \varrho \Bigg) + \frac{\pi}{L} \Bigg( \frac{1}{2} - \frac{(\tilde J_{s\bar h} + j_1)}{N}\Bigg) \Bigg( 1 + \frac{1}{c} \varrho \Bigg) + \ldots,  \\
q_L = \pi \varrho \Bigg( 1 - \frac{2}{c} \varrho \Bigg) - \frac{\pi}{L} \Bigg( \frac{1}{2} - \frac{(\tilde J_{s\bar h} + j_1)}{N}\Bigg) \Bigg( 1 + \frac{1}{c} \varrho \Bigg) + \ldots ,
\eea
which are slight modifications of the expansions found for the spinon dispersion, reflecting the hole in the Fermi sea of momenta integers. Here we have defined $\Xi(x)$ such that $\Xi(x<0) = -1$ and $\Xi(x\ge0) = 1$.  

\end{comment}
